Multiscale model reduction for incompressible flows

Many unsteady flows exhibiting complex dynamics are nevertheless characterized by emergent large-scale coherence in space and time. Reduced-order models based on Galerkin projection of the governing equations onto an orthogonal modal basis approximate the flow as a low-dimensional dynamical system with linear and quadratic terms. However, these Galerkin models often fail to reproduce the true dynamics, in part because they ignore important nonlinear interactions with unresolved flow scales. Here, we use a separation of time scales between the resolved and subscale variables to derive a reduced-order model with cubic closure terms for the truncated modes, generalizing the classic Stuart-Landau equation. The leading order cubic terms are determined by averaging out fast variables through a perturbation series approximation of the action of a stochastic Koopman operator. We show analytically that this multiscale closure model can capture both the effects of mean-flow deformation and the energy cascade before demonstrating improved stability and accuracy in models of chaotic lid-driven cavity flow and vortex pairing in a mixing layer. This approach to closure modeling establishes a general theory for the origin and role of cubic nonlinearities in low-dimensional models of incompressible flows

==> A4_Homogenization.tex <==
\appendix

\section{(Possible): Comparison to homogenization technique}
Consider the two-dimensional fast-slow system
\begin{subequations}
\begin{align}
    \dot{x} &= \epsilon^2 \lambda x - \beta xy \\
    \dot{y} &= -\nu y + \gamma x^2 + \epsilon \sigma w(t),
\end{align}
\end{subequations}
where $\epsilon \ll 1$ is a measure of distance from a bifurcation.
We therefore expect the slow amplitude to scale with $\epsilon$.
Let $x(t) = \epsilon a(\tau)$ with $\tau = \epsilon^2 t$, so that with the scaling properties of white noise the system becomes
\begin{subequations}
\begin{align}
    \dot{a} &= \lambda a - \epsilon^{-1} \beta ab \\
    \dot{b} &= -\epsilon^{-2}\nu b + \epsilon^{-1}\gamma a^2 + \epsilon^{-2} \sigma w(\tau).
\end{align}
\end{subequations}
This fast/slow SDE system is associated with the following backwards Kolmogorov equation (BKE) for an arbitrary scalar observable $g^\epsilon$:
\begin{equation}
\label{eq:toy-BKE}
    \partial_t g^\epsilon = \left\{ 
    \epsilon^{-2} \left[ -\nu b \pdv{b} + \frac{\sigma^2}{2} \pdv[2]{b} \right] + \epsilon^{-1} \left[ -\beta ab \pdv{a} + \gamma a^2 \pdv{b} \right] + \lambda a \pdv{a}
    \right\} g^\epsilon.
\end{equation}
Separating by powers of $\epsilon$, this is 
\begin{equation}
    \partial_t g^\epsilon = \left[
    \epsilon^{-2} \mathcal{L}_0 + \epsilon^{-1} \mathcal{L}_1 + \epsilon^{0}\mathcal{L}_2
    \right] g^\epsilon.
\end{equation}
Note that $\mathcal{L}_0$ is the backwards Kolmogorov operator associated with an Ornstein-Uhlenbeck process; the nonlinear term $\gamma a^2$ can be viewed as an $\mathcal{O}(\epsilon)$ perturbation to an Ornstein-Uhlenbeck process whose steady-state distribution $p(b)$ is given by the solution to the Fokker-Planck equation
\begin{equation}
\label{eq:toy-OU-FP}
    \mathcal{L}_0^\dagger p(b) = 0.
\end{equation}
The solution to this is the Gaussian distribution
\begin{equation}
    p(b) = \frac{\nu}{\pi \sigma^2} \exp \left[ -\frac{nu b^2}{\sigma^2} \right].
\end{equation}
We will assume that the BKE~\eqref{eq:toy-BKE} can be solved with the asymptotic expansion
\begin{equation}
    g^\epsilon = g_0 + \epsilon g_1 + \epsilon^2 g_2 + \dots.
\end{equation}
Substituting and equating powers of $\epsilon,$ the consistency conditions for the expansion are
\begin{subequations}
\begin{align}
    \label{eq:toy-order2}
    \mathcal{L}_0 g_0 &= 0 \\
    \label{eq:toy-order1}
    \mathcal{L}_0 g_1 &= -\mathcal{L}_1 g_0 \\
    \label{eq:toy-order0}
    \mathcal{L}_0 g_2 &= \partial_t g_0 - \mathcal{L}_1 g_1 - \mathcal{L}_2 g_0
\end{align}
\end{subequations}
with the operators
\begin{subequations}
\begin{align}
    \mathcal{L}_0 &= -\nu b \pdv{b} + \frac{\sigma^2}{2} \pdv[2]{b} \\
    \mathcal{L}_1 &= -\beta ab \pdv{a} + \gamma a^2 \pdv{b} \\
    \mathcal{L}_2 &= \lambda a \pdv{a}.
\end{align}
\end{subequations}
Each condition requires that the mean of the right hand side with respect to the OU distribution is zero.
To see this, evaluate this mean of the action of $\mathcal{L}_0$ with respect to an arbitrary observable $g$:
\begin{equation}
    \int_{-\infty}^{\infty} p(b) \mathcal{L}_0 g \dd b = \int_{-\infty}^{\infty} g \mathcal{L}_0^\dagger p(b) \dd b,
\end{equation}
which evaluates to zero by virtue of Eq.~\eqref{eq:toy-OU-FP}.

\begin{itemize}
    \item \textbf{Order} $\epsilon^{-2}$: Eq.~\eqref{eq:toy-order2} is trivially satisfied if $g_0 = g_0(a)$, or in other words if the asymptotic solution does not depend on the fast variable, as we expect.
    \item \textbf{Order} $\epsilon^{-1}$: The slow drift terms must have zero mean with respect to $p(b)$.
    In other words, all terms in the equation for $\dot{a}$ must be linear in $b$ so that the Gaussian integral vanishes by symmetry.
    The consistency condition is
    \begin{equation}
       -\beta ab \pdv{a} g_0 = -\left[ -\nu b \pdv{b} + \frac{\sigma^2}{2} \pdv[2]{b} \right] g_1,
    \end{equation}
    which is satisfied if
    \begin{equation}
        g_1 = -\frac{\beta}{\nu} ab \pdv{g_0}{a}
    \end{equation}
    \item \textbf{Order} $\epsilon^{0}$: With the $\mathcal{O}(\epsilon^{-1}$ solution, the requirement that the right-hand side have zero mean with respect to the OU distribution leads to a second backwards Kolmogorov equation which is averaged over the fast variables.
\end{itemize}

In particular, the consistency condition is that
\begin{subequations}
\begin{align}
    0 &= \int \left[ \partial_t g_0 - \mathcal{L}_1 g_1 - \mathcal{L}_2 g_0 \right] p(b) \dd b \\
    &= \partial_t g_0 - \int \mathcal{L}_1 g_1 p(b) \dd b - \int \mathcal{L}_2 g_0 p(b) \dd b.
\end{align}
\end{subequations}
After expanding and some rearranging, this becomes
\begin{equation}
    \partial_t g_0 = \left\{ \lambda a \pdv{a} + \frac{\beta^2}{\nu} a \left[ \int b^2 p(b) \dd b \right] \pdv{a} - \frac{\beta \gamma}{\nu} a^3 \pdv{a} + \frac{\beta^2}{\nu} a^2 \left[ \int b^2 p(b) \dd b \right] \pdv[2]{a} \right \} g_0.
\end{equation}
The Gaussian integral evaluates to
\begin{equation}
    \int b^2 p(b) \dd b = \frac{\sigma^2}{2 \nu},
\end{equation}
so the full asymptotic solution is
\begin{equation}
    \partial_t g_0 = \left\{ (\lambda + D) a \pdv{a} - \mu a^3 \pdv{a} + D a^2 \pdv[2]{a} \right \} g_0,
\end{equation}
with $D = \beta^2 \sigma^2 / 2 \nu^2$ and $\mu = \beta \gamma/ \nu$.
This is the backwards Kolmogorov equation corresponding to the slow-time Langevin equation
\begin{equation}
    \dot{a} = (\lambda + D)a - \mu a^3 + \sqrt{2D} a w(\tau).
\end{equation}
Finally, the scaling can be undone to recover the original coefficients, implying that there does not need to be an explicit $\epsilon$ parameter:
\begin{equation}
    \dot{x} = \epsilon^2(\lambda + D)x - \mu x^3 + \epsilon \sqrt{2D} x w(t).
\end{equation}
